Internal Neighbourhood Spaces

The main aim of this paper is to provide a description of neighbourhood operators in finitely complete categories with finite coproducts and a proper factorisation system such that the semilattice of admissible subobjects make a distributive complete lattice. The equivalence between neighbourhoods, Kuratowski interior operators and pseudo-frame sets is proved. Furthermore the categories of internal neighbourhoods is shown to be topological. Regular epimorphisms of categories of neighbourhoods are described and conditions ensuring hereditary regular epimorphisms are probed. It is shown the category of internal neighbourhoods of topological spaces is the category of bitopological spaces, while in the category of locales every locale comes equipped with a natural internal topology.

==> Factorisations_v2.tex <==
\section{Factorisation Systems and Admissible Subobjects}
\label{Factorisations}

The modern notion of a factorisation system
\opair{\mathsf{E}}{\mathsf{M}} was introduced in \cite{FreydKelly1972}.
The earlier {\em bicategorical structures} of Isbell (see
\cite{Isbell1964}) can be seen today as those factorisation systems where
every $\mathsf{E}$ is an epimorphism and each $\mathsf{M}$ is a
monomorphism. In this section the necessary facts for factorisation
systems are collected in the form given e.g. in \cite[\S 2]{Janel1997b}.

\input{prel-factsys}
\input{prel-admsubobjects}
